Assessing Exoplanetary System Architectures with DYNAMITE Including Observational Upper Limits

The information gathered from observing planetary systems is not limited to the discovery of planets, but also includes the observational upper limits constraining the presence of any additional planets. Incorporating these upper limits into statistical analyses of individual systems can significantly improve our ability to find hidden planets in these systems by narrowing the parameter space in which to search. Here I include radial velocity (RV), transit, and transit timing variation (TTV) upper limits on additional planets in known multi-planet systems into the DYNAMITE software package and test their impact on the predicted planets for these systems. The tests are run on systems with previous DYNAMITE analysis and with updated known planet parameters in the 2-3 years since the original predictions. I find that the RV limits provide the strongest constraints on additional planets, lowering the likelihood of finding them within orbital periods of ~10-100 days in the inner planetary systems, as well as truncating the likely planet size (radius and/or mass) distributions towards planets smaller than those currently observed. Transit and TTV limits also provide information on the size and inclination distributions of both the known and predicted planets in the system. Utilizing these limits on a wider range of systems in the near future will help determine which systems might be able to host temperate terrestrial planets and contribute to the search for extraterrestrial biosignatures.

==> reviewer_report.tex <==
REVIEWER COMMENT
The author has taken into account most of my comments. I only have the following minor suggestions:
----- AUTHOR RESPONSE -----
I thank the reviewer for the additional suggestions to improve the manuscript, and I have addressed them in the manuscript and below.

REVIEWER COMMENT
Lines 232: the effects may be small on short time scale but may have minutes variation on long time scale, e.g. https://iopscience.iop.org/article/10.3847/1538-4365/ad0847/pdf
So the authors may say that the time scale of these effects are much longer than the orbital periods of the targets and thus will not be considered. There is also a typo of in the sentence.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and have included the clarification about the time scale of the effects.

REVIEWER COMMENT
line 256-265: this sentence contains multiple brackets and is too long. I suggest rewording it using multiple short sentences.
----- AUTHOR RESPONSE -----
I agree with the reviewer and have reworded it into shorter sentences for clarity and ease of reading.

==> reviewer_report_v1.tex <==
REVIEWER COMMENT
This study utilizes RV, transit, and TTV observation upper limits with DYNAMITE to constrain additional planets in three systems. The probability of proposed planet candidates is evaluated using DYNAMITE analyses. This predictive work is essential for informing the detection and confirmation of additional planets and for narrowing down HWO targets. The research is promising and could be accepted for publication after addressing the following issues:
----- AUTHOR RESPONSE -----
I thank the reviewer for their report on how to improve the manuscript and agree that with the proposed changes to strengthen the paper. I have addressed all of the comments, and I detail those edits below.

REVIEWER COMMENT
Main Issues:

1. Section 2.1: The definition of RV upper limits is unclear. It varies depending on whether a planet candidate is subtracted from the RV data. For example, in the case of Tau Ceti, if planet b is not treated as a known planet, its signal should not be subtracted, leading to a higher RV upper limit.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and have expanded upon this point in Section 2.1, along with a reference to a method that has produced RV upper limits used in this analysis.

REVIEWER COMMENT
2. Section 2.3: The TTV upper limit procedure does not consider effects such as apsidal precession, the Rømer effect, and the Applegate effect. The current analysis is restricted to resonance effects.
----- AUTHOR RESPONSE -----
I agree with the reviewer's comment and have expanded on this choice in the text, stating that resonance effects provide the strongest signals with the current timespans, as well as apsidal precession is strongest with hot Jupiters, the Rømer effect of finite light travel time is << 1 second for these planetary masses and orbital periods, and the Applegate effect is most significant over long (multi-year) timescales.

REVIEWER COMMENT
3. RV, TTV, and Transit Upper Limits: These limits depend on both amplitude and timespan. While the analysis focuses on planets with orbital periods shorter than the data timespan, it is crucial to note that this technique is not applicable for longer periods.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and have clarified this point in the beginning of Section 2.

REVIEWER COMMENT
4. Section 2.2: The planet radius upper limit is used instead of the transit depth upper limit. Transit light curves cannot provide a radius limit due to the impact factor dependence; large planets with high impact factors can be missed. Consider the differences in signal-to-noise ratio for short and long-period transiting planets.
----- AUTHOR RESPONSE -----
I thank the reviewer for this clarification and have adjusted the text to describe how the upper limit is on the transit depth, and how when that gets translated to planet radius the large planets with high impact factors can be missed. Also, I have discussed the SNR for different-period transiting planets

REVIEWER COMMENT
5. Section 3: Include a summary paragraph in each subsection discussing the probability of proposed planet candidates or additional planets for clearer system analysis, given the numerous variations in the setups.
----- AUTHOR RESPONSE -----
I agree with the reviewer's comment and have added a summary paragraph in each subsection for clearer system analysis.

REVIEWER COMMENT
Minor Issues:

Line 103: Explain why astrometry and direct imaging are not considered in the upper limits.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and now note later in the paragraph that direct imaging limits are currently feasible for a different population and astrometry limits from future Gaia releases is the standard, so both will be included eventually but are not as universally applicable as RV, transit, and TTV limits are currently.

REVIEWER COMMENT
Lines 122-124: Clarify if dynamical instability is considered in the likelihood calculation; if not, explain why.
----- AUTHOR RESPONSE -----
I agree with the reviewer that clarifying the dynamical stability is considered in the new likelihood calculations with the upper limits and have addressed that in the text.

REVIEWER COMMENT
Lines 193-199: The assumption of zero longitude of the ascending node is strong and needs more justification.
----- AUTHOR RESPONSE -----
I agree with the reviewer about this comment and have found that this is a bit too strong of an assumption without checking it in the analysis, so I re-did the analysis without that assumption and allowing it to be a random angle, which did not significantly affect the final results but is still a more accurate treating of the situation. The text has been updated to reflect this change.

REVIEWER COMMENT
Lines 207-212: Specify the REBOUND setup, including the time span and time steps of the simulations.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and have specified the original setup of the REBOUND N-body integrations.

REVIEWER COMMENT
Lines 426-429: Justify why the outer planet is not considered and why it doesn't influence inner planet stability. Include it in analyses to verify your statement.
----- AUTHOR RESPONSE -----
I agree with the reviewer on this comment and have included it in the analyses, and I have updated the text to remove this assumption and the figures to show that the planet is included.

REVIEWER COMMENT
Figures 1-2, and others: Explain why the habitable zone in each figure is period-dependent.
----- AUTHOR RESPONSE -----
I thank the reviewer for this comment and have clarified in the first figure (and referred to it in subsequent figures) that the habitable zone is age- and period-dependent due to the evolution of the host star.
